Towards an End-to-End (E2E) Adversarial Learning and Application in the Physical World

The traditional learning process of patch-based adversarial attacks, conducted in the digital domain and then applied in the physical domain (e.g., via printed stickers), may suffer from reduced performance due to adversarial patches' limited transferability from the digital domain to the physical domain. Given that previous studies have considered using projectors to apply adversarial attacks, we raise the following question: can adversarial learning (i.e., patch generation) be performed entirely in the physical domain with a projector? In this work, we propose the Physical-domain Adversarial Patch Learning Augmentation (PAPLA) framework, a novel end-to-end (E2E) framework that converts adversarial learning from the digital domain to the physical domain using a projector. We evaluate PAPLA across multiple scenarios, including controlled laboratory settings and realistic outdoor environments, demonstrating its ability to ensure attack success compared to conventional digital learning-physical application (DL-PA) methods. We also analyze the impact of environmental factors, such as projection surface color, projector strength, ambient light, distance, and angle of the target object relative to the camera, on the effectiveness of projected patches. Finally, we demonstrate the feasibility of the attack against a parked car and a stop sign in a real-world outdoor environment. Our results show that under specific conditions, E2E adversarial learning in the physical domain eliminates the transferability issue and ensures evasion by object detectors. Finally, we provide insights into the challenges and opportunities of applying adversarial learning in the physical domain and explain where such an approach is more effective than using a sticker.

==> sections/acknowledgment.tex <==
\section*{Acknowledgment}

==> sections/countermeasure.tex <==
\section{Projection Detection}
\label{sec:countermeasure}

In this section, we focus on the development of a countermeasure to detect unauthorized projections on objects. This section details the process of training a classifier that effectively identifies projections on objects, which can be useful in mitigating the impact of adversarial patch attacks projected on objects.

\begin{figure} 
	\centering
	\includegraphics[width=0.98\linewidth]{figs/classifier_pipeline.png}
	\caption{Integration of the classifier into the object detection pipeline. The classifier analyzes each frame to detect projected adversarial patches. If a patch is detected, an alert is generated, and the frame is flagged as suspicious. If no patch is detected, the frame proceeds to the object detection system.}
	\label{fig:classifier_pipeline}
\end{figure}

\subsection{Goal} 
The primary goal is to develop a robust classifier that distinguishes between frames with and without projected adversarial patches.
As illustrated in Figure \ref{fig:classifier_pipeline}, the proposed classifier can be integrated into the preprocessing pipeline, analyzing each frame before the object detection system processes it.
By accurately detecting these projections, we can significantly enhance the resilience of object detection systems against adversarial attacks that exploit projected patches.

\subsection{Data Collection and Preprocessing}
\label{subsec:data_preproccessing}

To train the classifier, we collected a dataset comprising two classes of images: \textit{patched objects} and \textit{unpatched objects}. 
The dataset includes 338 images with patches projected onto objects and 324 images of objects without projected patches, captured from various angles and distances, and under different lighting conditions. 
A total of X different types of objects were included in the photo scenes, covering various categories such as cars, stop signs, and more.
The preprocessing steps involved rescaling pixel values to the [0, 1] range and applying data augmentation techniques to increase variability and robustness.
Specifically, the data augmentation techniques, include rotation, width and height shifts, zooming, and horizontal flipping.

\subsection{Model Architecture}
We designed a Convolutional Neural Network (CNN) tailored for the binary classification task of detecting projected patches. 
The model consists of several convolutional layers, followed by max-pooling layers, a flattening layer, dense layers, and a final sigmoid activation function for binary classification.
Additionally, we employed L2 regularization and used the Adam optimizer with a learning rate of 1e-4.

\subsection{Training Process}
The model was trained using the training dataset mentioned in Subsection \ref{subsec:data_preproccessing}, with 80\% of the data used for training and 20\% reserved for validation. The training process involved the following steps:
\begin{itemize}
\item Data Generators: Creation of data generators for training and validation sets with the specified augmentations and rescaling.
\item Model Compilation: Compiling the model with binary cross-entropy loss and monitoring accuracy and AUC metrics.
\item Callbacks: Utilizing ModelCheckpoint to save the best-performing model and EarlyStopping to halt training if the validation loss did not improve for 100 epochs.
\end{itemize}

\subsection{Model Evaluation}
Add here plots of the ROC curve, confusion matrix, training, and validation accuracy/loss.
Mention the final metrics (accuracy, AUC) on the validation set.

==> sections/tables/transferability-table-analysis3.tex <==
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{ % This resizes the table to fit the column width
\begin{tabular}{@{}ccccccc@{}}
\toprule
\textbf{Attack Type}             & \textbf{Target Detector}              & \textbf{Target Object}        & \begin{tabular}[c]{@{}c@{}}\textbf{Clean Detection Score}\\  \textbf{(Target Object)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Patched Detection Score}\\ \textbf{(Target Object)}\end{tabular} & \textbf{Tested Object} & \begin{tabular}[c]{@{}c@{}}\textbf{Percentage Confidence Difference} \\ \textbf{Between Clean \& Patched Objects}\end{tabular} \\ \midrule
\multirow{4}{*}{DPatch} & \multirow{4}{*}{YOLOv3}      & \multirow{4}{*}{Car} & \multirow{4}{*}{0.99}                                                            & \multirow{4}{*}{0.15}                                                             & Stop Sign     & 0\%                                                                                                                  \\
                        &                              &                      &                                                                                  &                                                                                   & Cup           & 0\%                                                                                                                  \\
                        &                              &                      &                                                                                  &                                                                                   & Bottle        & 0\%                                                                                                                  \\
                        &                              &                      &                                                                                  &                                                                                   & Potted Plant  & 0\%                                                                                                                  \\ \midrule
\multirow{4}{*}{NAP}    & \multirow{4}{*}{Faster-RCNN} & \multirow{4}{*}{Car} & \multirow{4}{*}{0.99}                                                            & \multirow{4}{*}{0}                                                                & Stop Sign     & 0\%                                                                                                                  \\
                        &                              &                      &                                                                                  &                                                                                   & Cup           & 0.78\%                                                                                                               \\
                        &                              &                      &                                                                                  &                                                                                   & Bottle        & 0\%                                                                                                                  \\
                        &                              &                      &                                                                                  &                                                                                   & Potted Plant  & 4.83\%                                                                                                               \\ \bottomrule
\end{tabular}
}
\caption{Transferability of Physical-Physical Patches: Impact on non-target objects when patch is designed for car detection}
\label{table:transferability-table-analysis3}
\end{table}

